LookWhere? Efficient Visual Recognition by Learning Where to Look and What to See from Self-Supervision

Vision transformers are ever larger, more accurate, and more expensive to compute. The expense is even more extreme at high resolution as the number of tokens grows quadratically with the image size. We turn to adaptive computation to cope with this cost by learning to predict where to compute. Our LookWhere method divides the computation between a low-resolution selector and a high-resolution extractor without ever processing the full high-resolution input. We jointly pretrain the selector and extractor without task supervision by distillation from a self-supervised teacher, in effect, learning where and what to compute simultaneously. Unlike prior token reduction methods, which pay to save by pruning already-computed tokens, and prior token selection methods, which require complex and expensive per-task optimization, LookWhere economically and accurately selects and extracts transferrable representations of images. We show that LookWhere excels at sparse recognition on high-resolution inputs (Traffic Signs), maintaining accuracy while reducing FLOPs by up to 34x and time by 6x. It also excels at standard recognition tasks that are global (ImageNet classification) or local (ADE20K segmentation), improving accuracy while reducing time by 1.36x. See https://github.com/antofuller/lookwhere for the code and weights.

==> extra.tex <==
INTRO

High-resolution imagery is now widely available in domains such as medical imaging, remote sensing, and consumer photography, with modern devices routinely capturing images at tens of megapixels.
These images offer rich, fine-grained visual detail that can significantly enhance the performance of computer vision models.
However, due to the high computational and memory costs associated with processing such data, they are often downsampled or discarded.
Vision Transformers (ViTs) [] have become a widely adopted architecture for various tasks in computer vision such as classification [], segmentation [], and object detection [], largely owing to their ability of modeling global context via self-attention.
Yet, this same self-attention mechanism incurs quadratic complexity in the number of tokens.
For many real-world applications with limited computational budgets or high-throughput requirements, sequence length therefore becomes a bottleneck; further compounded by trends toward finer tokenizations [patch-size=1 papers], higher-resolution inputs [DPS, IPS], and larger model sizes [], rendering full-resolution processing increasingly impractical in real-world, resource-constrained settings.
Although these limitations seem to preclude scaling to higher resolutions, a glimmer of hope arises from the fact that natural images exhibit substantial \textbf{spatial redundancy}---neighboring pixels are highly spatially correlated, and larger regions often contain repetitive patterns or non-salient backgrounds.
This redundancy therefore raises an important question: \textit{can we drop patches to save computation}?

Recent work suggests the answer is yes---selectively dropping image patches can lead to more compact and efficient image representations.
Accordingly, various strategies for token reduction have been proposed to progressively shorten sequence lengths as inputs pass through transformer layers.
These methods generally fall into one of two categories: token \textit{pruning} and token \textit{merging}.
The former seeks to discard uninformative tokens, which may be achieved by retraining the network to dynamically filter tokens using learnable masks guided by predefined metrics [], or by learning a policy to retain only the most relevant tokens [].
Conversely, token merging reduces redundancy by combining semantically similar tokens rather than discarding them. Similarity can be estimated via class token attention scores [], comparing key vectors from self-attention [], or more recently, through clustering-based approaches [].
Despite the clear computational savings both these approaches offer, they still share a fundamental limitation in still requiring \textit{all} tokens to be processed for a number of initial layers in order to determine which tokens may be dropped.
This full-token processing fails to scale with finer tokenizations, and is particularly problematic for high-resolution inputs, often leading to out-of-memory errors.
Evaluating every token to decide whether it may be dropped introduces additional overhead; ideally, irrelevant tokens should be recognized quickly and discarded early to maximize efficiency which raises our next question: \textit{can we efficiently recognize redundant patches, and avoid full-token processing in early layers altogether?}

Encouragingly, the answer is positive once again.
A naive approach might involve randomly dropping patches, or downsampling the entire image to reduce the patch count.
However, random dropping risks removing patches critical to the task, while downsampling can obscure fine-grained details resulting in performance degredation.
Hence, effective patch selection must i) account for patch semantics to discard only uninformative regions, while ii) retaining the ability to process important fine details.
Since full-resolution analysis is prohibitively expensive, alternative works have proposed methods that operate on reduced or partial image views to guide selective refinement---an approach that may be framed as \textit{zooming}.
The model must decide---given a constrained representation---which patches are sufficiently salient to warrant more detailed analysis, effectively `zooming in' on the most informative regions. In [] and [], the input is down-scaled to a lower-resolution and a differentiable selection process is used to select the most relevant low-res patches for subsequent high-res processing [DPS, PD]. Instead of down-scaling, [IPS] processes subsets of patches from the input iteratively, and maintains the top most salient patches for subsequent processing. 
Both methods generally train end-to-end, through supervised learning, to recognize informative patches; the model is simultaneously trained to select patches and perform the task with its selection. As a result, learning tends to select patches that are less likely to hurt task performance, leading to a task-specific inductive bias. The model may then remove image patches containing useful semantics, but are not captured by any learned category. To mitigate such task-specific bias, [LTRP] employs a self-supervised reconstruction objective. A pretrained masked autoencoder is used to generate pseudo-labels representing patch importance, which are then used to train a model that predicts these semantic patch rankings.

While this approach helps decouple patch selection from specific downstream tasks, it only addresses one part of the zooming problem. Namely, it does not train a model that can \textit{use} these sparse representations for arbitrary downstream tasks. The full `zooming' system---comprising both patch selection and finer downstream processing---is still trained in a task-specific manner and is unlikely to generalize across tasks. In the era of the Vision Transformer, which benefits significantly from pretraining on massive unlabeled data [], it is desirable to develop a zooming mechanism that can be pretrained end-to-end and later fine-tuned for various downstream applications.

To tackle this challenge, we introduce \textit{LookWhere}, a framework for pretraining a general-purpose zooming model using self-supervised token distillation. Our method leverages salient attention maps from a pretrained DINOv2 model to train a patch selection \textit{zoomer}, and employs a latent reconstruction objective---based on DINO’s learned visual features---to train the model to recover image representations from sparse high-resolution inputs. Through extensive experiments, we fine-tune LookWhere and compare it to state-of-the-art zooming and token reduction techniques. We show that LookWhere (i) improves performance on classification, segmentation, and object recognition tasks, and (ii) offers a competitive solution for efficient ViTs and scaling to larger architectures. We further analyze LookWhere, finding...

==> main_figure/architecture.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{main_figure/architecture2.pdf}
\caption{LookWhere uses}
\label{fig:trq-dia}
\end{figure*}  

==> oracle/wrapper_old.tex <==
\begin{figure}[!htb]
  \centering
  % scale everything inside by 0.9x
  \scalebox{0.75}{%
    \noindent
    % left box (top-aligned)
    \begin{minipage}[c]{0.45\textwidth}
      \centering
      \input{oracle/classification_k=128}
      % \par
      % \vspace*{0.1cm}
      \input{oracle/segmentation_k=128}
    \end{minipage}
    \hspace{2cm}
    % right box (also top-aligned)
    \begin{minipage}[c]{0.45\textwidth}
      \centering
      \vspace*{0.1cm}
      \textbf{Which attention map should\\ \quad \quad the selector target?}
      \vspace*{0.1cm}
      \input{oracle/attention_target_blocks}
    \end{minipage}%
  }
  \caption{%
  When used as a selector map, the \textbf{last} layer's \textcolor{pat_color}{patch} queries achieve the best balance between classification and segmentation (\textcolor{lwcolor}{shaded}). We thus train our selector to predict this attention map during distillation pretraining. For classification ($k$NN with $k{=}128$ on ImageNet-HR), \textbf{deeper} attention maps and \textcolor{cls_color}{class} queries generally perform best. For segmentation ($k$NN with $k{=}128$ on ADE20K), averaging over \textbf{all} layers and \textcolor{pat_color}{patch} queries generally perform best.
  }
  \label{fig:combined}
\end{figure}


==> results/imagenet_older.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{%
    \textbf{Image Classification on ImageNet.} 
    LookWhere is more accurate and significantly faster than SoTA adaptive computation methods for ViTs.
    % and is significantly faster.
    % LookWhere outperforms SoTA token reduction methods and is significantly faster.
    % PiToMe does not report ViT-Base results and LTRP does not report ViT-Small results.
    DINO-v2 is a non-adaptive baseline: it reaches the highest accuracy but at the highest FLOPs.
    % All models are finetuned on ImageNet-1K at $224^2$ px resolution.
    % DPS and IPS are not benchmarked on ImageNet, as they are specialized for high resolution. 
    Inference memory is equal for all models.
    }
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{lccc|cccc}
        \toprule
        Method & \makecell{Top-$1$ Acc.\\$\%$ $\uparrow$} 
         & \makecell{FLOPs\\G $\downarrow$} & \makecell{Speed\\K im/s $\uparrow$} & \makecell{Top-$1$ Acc.\\$\%$ $\uparrow$} & \makecell{FLOPs\\G $\downarrow$}  & \makecell{Speed\\K im/s $\uparrow$}\\
         \midrule
            & \multicolumn{3}{c}{\emph{ViT-Small architectures}} & \multicolumn{3}{c}{\emph{ViT-Base architectures}}\\
            DINOv2 \cite{oquab2023dinov2} & $81.9$ & $6.2$ & $6.8$ & $84.2$ & $23.6$ & $2.2$\\ 
            % DINOv2 \cite{oquab2023dinov2} ($224^2$) & X & X & X & $6.8$ & X & X & X & $2.2$\\ 
            % DINOv2 \cite{oquab2023dinov2} ($182^2$) & X & X & X & $10.7$ & X & X & X & $3.5$\\ 
            \midrule
            PiToMe \cite{tran2024pitome} {\tiny ($r$=$0.925$)} & $79.8$/- & $3.1$/- & $6.6$/- & - & - & -\\ 
            DTEM \cite{lee2024dtem} {\tiny ($r$=$16$)} & $79.4$/$80.7$ & $2.4$/$9.2$ & $7.0$/$3.8$ & $80.7$ & $9.2$ & $3.8$  \\ 
            ATC \cite{haurum2024atc} {\tiny ($r$=$0.9$)} & $79.9$/$82.0$ & $4.0$/$15.3$ & $0.4$/$0.4$ & $82.0$ & $15.3$ & $0.4$ \\
            LTRP \cite{luo2024learning} {\tiny ($keep$=$0.75$)} & -/$82.8$ & -/$18.3$ & -/$2.3$ & -/$82.8$ & -/$18.3$ & -/$2.3$ \\
            % \rowcolor{lowcolor!10} LookWhere ($k$=$64$)  & X & $2.3$ & $0.1$ & $10.0$ & $81.7$ & $9.1$ & $0.4$ & $4.7$ \\
            \rowcolor{lwcolor!10} \textbf{LookWhere} {\tiny ($k$=$128$)} & $80.3$/$83.0$  & $3.8$/$14.8$ & $9.5$/$3.2$ & $83.0$ & $14.8$ & $3.2$\\
         \bottomrule
    \end{tabular}
    \label{tab:imagenet}

\end{table}

==> results/imagenet_stacked.tex <==
\begin{table}[ht]
    \centering
    \small
    \caption{%
    \textbf{ImageNet results.} 
    LookWhere outperforms SoTA token reduction methods and is significantly faster.
    All models are finetuned on ImageNet-1K at $224^2$ px resolution.
    PiToMe does not report ViT-Base results and LTRP does not report ViT-Small results.
    \es{Please move accuracy to the left. For space ViT-Small and ViT-Base should be side-by-side, not stacked.}
    }
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lccccc}
        \toprule
        Method & \makecell{Top-$1$ Acc.\\$\%$} 
         & \makecell{FLOPs\\G} & \makecell{Memory\\GB} & \makecell{Speed\\K imgs/s} \\
         \midrule
            \multicolumn{5}{c}{\emph{ViT-Small architectures}}\\
            PiToMe \cite{tran2024pitome} & $79.8$ & $3.1$ & $0.2$ & $6.6$ \\ 
            DTEM \cite{lee2024dtem} & $79.4$ & $2.4$ & $0.2$ & $7.0$ \\ 
            ATC \cite{haurum2024atc} & $79.9$ & $4.0$ & $0.2$ & $0.4$ \\

            \rowcolor{lowcolor!10} LookWhere ($k$=$128$) & $80.3$  & $3.8$ &  $0.2$ & $9.5$ \\
            \midrule
            \multicolumn{5}{c}{\emph{ViT-Base architectures}}\\
            DTEM \cite{lee2024dtem} & $80.7$ & $9.2$ & $0.5$ & $3.8$ \\
            ATC \cite{haurum2024atc} & $82.0$ & $15.3$ & $0.5$ & $0.4$ \\
            LTRP \cite{luo2024learning} & $82.8$ & X & X & X \\
            \rowcolor{lowcolor!10} LookWhere ($k$=$72$) & $81.7$ & $9.9$ & $0.5$ & $4.7$ \\
            \rowcolor{lowcolor!10} LookWhere ($k$=$92$) & $82.5$ & $11.6$ & $0.5$ & $4.0$ \\
            \rowcolor{lowcolor!10} LookWhere ($k$=$128$) & $83.0$ & $14.8$ & $0.5$ & $3.2$ \\
         \bottomrule
    \end{tabular}
    \label{tab:bonus_bonus}

\end{table}

==> results/traffic_full.tex <==
\begin{table}[ht]
  \centering
  \caption{Traffic}
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{llcccccccccc} 
    \toprule
    & Res. 
    & \multicolumn{4}{c}{Top-1 Acc. (by LR)}
    & \multicolumn{3}{c}{Train}
    & \multicolumn{3}{c}{Eval} \\
    \cmidrule(lr){3-6}
    \cmidrule(lr){7-9}
    \cmidrule(lr){10-12}
    & & $2$e-$5$ & $5$e-$5$ & $8$e-$5$ & $1$e-$4$ 
    & Spd & Mem. & FLOPs
    & Spd & Mem. & FLOPs \\
    \midrule
    \multirow{1}{*}{PiToMe []} 
      % & $518$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      % & $700$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      & $994$ & -- & -- & -- & -- & 48.1 & 4.2 & 1318 & 108.8 & 6.8 & 342 \\
    \midrule
    \multirow{1}{*}{ATC []} 
      % & $518$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      % & $700$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      & $994$ & -- & -- & -- & -- & 1.1 & 20.0 & 1507 & 1.3 & 6.6 & 389 \\
    \midrule
    \multirow{1}{*}{DTEM []} 
      % & $518$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      % & $700$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      & $966$ & -- & -- & -- & -- & OOM & OOM & OOM & 27.4 & 11.6 & 395 \\
    \midrule
    \multirow{1}{*}{DPS []} 
      & $980$ & 53.5 & 82.6 & 83.6 & 78.21 & 34.2 & 4.1 & 147 & 287.8 & 2.4 & 48 \\
    \midrule
    \multirow{1}{*}{IPS []} 
      & $980$ & -- & -- & -- & -- & 36.15 & 3.5 & 1540 & 74.9 & 2.4 & 514 \\
    \midrule
    \multirow{1}{*}{Plain ViT-S []} 
      % & $518$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      % & $700$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      & $994$ & -- & -- & -- & -- & 7.5 & 18.6 & OOM & 23.5 & 3.6 & 691 \\
    \midrule
    \multirow{1}{*}{\textbf{LookWhere (ours)}} 
      % & $518$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      % & $700$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      & $994$ & 93.4 & 90.6 & 95.2 & 91.5 & 48.2 & 3.6 & 331 & 243.5 & 2.2 & 91 \\
    \bottomrule
  \end{tabular}
  \label{tab:univariate}
\end{table}

==> results/traffic_old.tex <==
\begin{table}[ht]
  \centering
  \caption{Traffic}
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{llcccccccccc} 
    \toprule
    & Res. 
    & \multicolumn{4}{c}{Top-1 Acc. (by LR)}
    & \multicolumn{2}{c}{Speed (K imgs/s)}
    & \multicolumn{2}{c}{Memory (GB)}
    & \multicolumn{2}{c}{FLOPs (G)} \\
    \cmidrule(lr){3-6}
    \cmidrule(lr){7-8}
    \cmidrule(lr){9-10}
    \cmidrule(lr){11-12}
    & & $2$e-$5$ & $5$e-$5$ & $8$e-$5$ & $1$e-$4$ 
    & Train & Eval 
    & Train & Eval 
    & Train & Eval \\
    \midrule
    \multirow{3}{*}{PiToMe []} 
      & $518$ & $64.3$ & $64.0$ & $62.7$ & $66.4$ & -- & -- & -- & -- & -- & -- \\
      & $700$ & $65.4$ & $62.4$ & $62.7$ & $65.5$ & -- & -- & -- & -- & -- & -- \\
      & $910$ & $67.5$ & $67.1$ & $68.6$ & $68.6$ & -- & 191.3 & -- & 3.4 & -- & 123.5 \\
    \midrule
    \multirow{3}{*}{ATC []} 
      & $518$ & $63.6$ & $64.3$ & $64.0$ & $69.3$ & -- & -- & -- & -- & -- & -- \\
      & $700$ & $63.6$ & $66.4$ & $66.2$ & $64.9$ & -- & -- & -- & -- & -- & -- \\
      & $910$ & $65.1$ & $65.1$ & $64.5$ & $64.8$ & -- & 2.2 & -- & 3.3 & -- & 139.3 \\
    \midrule
    \multirow{3}{*}{DTEM []} 
      & $518$ & $82.3$ & $87.7$ & $85.8$ & $81.7$ & -- & -- & -- & -- & -- & -- \\
      & $700$ & $86.8$ & $83.6$ & $90.0$ & $82.9$ & -- & -- & -- & -- & -- & -- \\
      & $700$ & $86.8$ & $83.6$ & $90.0$ & $82.9$ & -- & -- & -- & -- & -- & -- \\
      & $910$ & $87.0$ & $94.7$ & $91.3$ & $87.7$ & -- & 68.2 & -- & 4.9 & --  & 141.6 \\
    \midrule
    \multirow{1}{*}{DPS []} 
      & $980$ & $65.2$ & $81.6$ & $77.3$ & $76.0$ & 245.1 & 290.6 & -- & 1.9 & -- & 14.0 \\
    \midrule
    \multirow{1}{*}{IPS []} 
      & $980$ & $86.6$ & $95.4$ & $94.1$ & $89.6$ & -- & 81.3 & -- & 1.6 & -- & 130.6 \\
    \midrule
    \multirow{3}{*}{Plain ViT-S []} 
      & $518$ & $82.9$ & $85.1$ & $89.0$ & $68.3$ & -- & -- & -- & -- & -- & -- \\
      & $700$ & $90.5$ & $92.3$ & $85.8$ & $86.1$ & -- & -- & -- & -- & -- & -- \\
      & $910$ & $89.3$ & $95.0$ & $90.3$ & $90.8$ & -- & 71.0 & -- & 2.4 & -- & 255.9 \\
    \midrule
    \multirow{3}{*}{\textbf{LookWhere (ours)}} 
      & $518$ & $78.2$ & $76.2$ & $80.0$ & $74.4$ & -- & -- & -- & -- & -- & -- \\
      & $700$ & $84.6$ & $84.5$ & $81.3$ & $84.3$ & -- & -- & -- & -- & -- & -- \\
      & $910$ & $87.2$ & $90.0$ & $86.7$ & $85.5$ & -- & 288.1 & -- & 2.2 & -- & 26.5 \\
    \bottomrule
  \end{tabular}
  \label{tab:univariate}
\end{table}

==> vary_k_and_random/figure.tex <==
% \begin{figure*}[!t]
% \hspace{0.1cm}
\centering
\input{vary_k_and_random/plot}
\caption{\textbf{Randomly selecting high-res patches reduces performance} by $2.1\%$ on ImageNet compared to our pretrained selector map. Varying $k$ offers flexibility at a small cost.
}
\label{fig:vary_k_random}
% \end{figure*}

==> zoom_example/zoom_figure.tex <==
\def\imgwidth{0.1825\textwidth}
\begin{wrapfigure}[20]{r}{0.56\textwidth}
    \centering
    \vspace{-10pt} 

    % --- First row: Traffic ---
    \parbox{\imgwidth}{
        \centering
        high-res input\\
        \includegraphics[width=\imgwidth]{zoom_example/original_image_traffic.pdf}
    }
    \parbox{\imgwidth}{
        \centering
        selector map\\
        \includegraphics[width=\imgwidth]{zoom_example/zoom_map_traffic_old.pdf}
    }
    \parbox{\imgwidth}{
        \centering
        sparse patches\\
        \includegraphics[width=\imgwidth]{zoom_example/topk_image_traffic.pdf}
    }

    \vspace{0.2cm}

    % --- Second row: Bird ---
    \parbox{\imgwidth}{
        \includegraphics[width=\imgwidth]{zoom_example/original_image_bird.pdf}
    }
    \parbox{\imgwidth}{
        \includegraphics[width=\imgwidth]{zoom_example/zoom_map_bird_old.pdf}
    }
    \parbox{\imgwidth}{
        \includegraphics[width=\imgwidth]{zoom_example/topk_image_bird.pdf}
    }
    \caption{%
    \textbf{Adaptively selected computation}. We visualize the selector’s prediction of \textit{where} to compute, alongside the extractor's sparse input that determines \textit{what} to see. The top depicts traffic sign recognition, while the bottom shows fine-grained bird classification.
    }
    \label{fig:selector_example}
\end{wrapfigure}
